How quantum computing can enhance biomarker discovery

Biomarkers play a central role in medicine's gradual progress towards proactive, personalized precision diagnostics and interventions. However, finding biomarkers that provide very early indicators of a change in health status, for example for multi-factorial diseases, has been challenging. Discovery of such biomarkers stands to benefit significantly from advanced information processing and means to detect complex correlations, which quantum computing offers. In this perspective paper, quantum algorithms, particularly in machine learning, are mapped to key applications in biomarker discovery. The opportunities and challenges associated with the algorithms and applications are discussed. The analysis is structured according to different data types - multi-dimensional, time series, and erroneous data - and covers key data modalities in healthcare - electronic health records (EHRs), omics, and medical images. An outlook is provided concerning open research challenges.

==> QML-snapshot.tex <==
Based on a reading of the paper, here are the QC Terms/concepts mentioned that need to be incorporated into the Quantum COmputing and QML sections in the intro.

QC Terms:
QPU: define by analogy to CPU and GPU
QRAM: look at current definition and conversation and determine if sufficient or need more context.
QGANs: decide if you want to expand/introduce QGANs in the QML Section.
QTDA: need a short section introducing QTDA.
Quantum Reservoir Computing: Do we need to introduce and define its approach.
QPCA: need a couple of sentences introducing QPCA.

Section 3: Mentions a number of QC concepts that we should introduce earlier or not mention at all.
Hilbert space
Quantum Device Connectivity
Error Mitigation Protocols

Numan will tackle editing the QML section to make sure that it's more in line with the paper.

Karl will edit the Quantum Computing section to make sure that whatever concepts are introduced in the paper are introduced and scoped correctly to the What is QC goal of the QC Section.


Karl: I have tried to incorporate the above already in the QC section since this is very general for qauntum computing.Please have a look. 

\section{Quantum computing}
\label{sec:qc}

Quantum computing is a relatively young field of research, undergoing rapid and substantial developments. Leveraging the fundamental properties of quantum mechanics, namely superposition and entanglement, Quantum Computing offers the exciting possibility to solve problems more efficiently than classical computers.  However, currently available quantum computers are prone to errors and face limitations in both the number of logical qubits (quantum bits) and the connectivity between them, both of which are essential to implement and correctly execute any algorithm. These constraints also introduce challenges in developing algorithms to achieve a quantum advantage with available quantum devices, commonly referred to as NISQ (Noisy Intermediate-Scale Quantum) hardware. Consequently,considerable efforts are being directed towards utilizing NISQ devices, while the development of noise-free, fault-tolerant, quantum hardware continues. 

Fault-tolerant quantum algorithms, such as Shor's RSA encryption breaking algorithm, typically require running deep circuits on tens of thousands to millions of logical qubits, making them unsuitable for near-term NISQ devices. On the other hand, variational quantum algorithms (VQAs)~\cite{cerezo_variational_2021} utilize shallower circuits and can produce meaningful results with error mitigation techniques. This characteristic has made VQAs highly popular for near-term quantum computing applications. VQAs are hybrid quantum-classical algorithms that involve an iterative loop between classical and quantum hardware. First, parameterized quantum circuits, called the ans\"atze, are employed to obtain samples from a quantum device. Then, a classical computer optimizes the parameters of the quantum circuit with respect to the loss function of the problem, see fig.~\ref{fig:quantum_pipeline}. The mathematical structure of VQAs bears resemblance to how Artificial Neural Networks are trained in Deep Learning, and as such, Quantum Machine Learning is one of the most common applications of NISQ hardware. 

In quantum computing, algorithms execute operations in Hilbert space, which is a high dimensional vector space, representing the state of qubits and is naturally suited to computing outcome probabilities (via an inner product). The essential feature of a Hilbert space is its exponenetial growth with with the number of qubits. This feature is essential to quantum computing's distinct potential advantages, where quantum circuits are executed in exponentially larger vector spaces, yet requiring only a polynomial increase in the number of qubits. The final execution is performed on Quantum hardware through 
Quantum Processor Units (QPUs), in analogy to CPUs or GPUs on classical digital computers or graphic cards. Another element is the Quantum Random Access Memory (QRAM), which is a quantum memory that stores a quantum state for later retrieval. Unlike QPUs which are readily available via Cloud computing platforms, hardware incorporating QRAM devices has not been demonstrated yet. 

Bringing all these characteristics of quantum computing together allows to perform already today first benchmark problems which serve to probe the power of quantum computing and pave the the way for future larger scale computations, which can lead eventually to a quantum advantage. 


\begin{figure}[h]%
\centering
\includegraphics[width=\linewidth]{figures/pipeline.pdf}
\caption{Workflow of data analysis using quantum computing}
\label{fig:quantum_pipeline}
\end{figure}

%Maria - should we add a box with definitions, e.g. quantum circuit, qubit, gate, entanglement, data embeddings..., maybe we should have appendix for this

\subsection{Quantum machine learning}

The domain of quantum machine learning (QML) integrates principles from quantum computing and machine learning, promising potential advances in learning from data. Learning from classical data typically requires data embedding into Hilbert space as the first step in quantum analysis pipeline. Analyzing high-dimensional classical datasets with quantum computing methods is challenging with near term devices. While there are various ways to embed classical data into quantum states, the number of available qubits is restricting the feature space size we can tackle with current devices. For instance, angle encoding~\cite{schuld2018supervised} or instantaneous quantum polynomial (IQP) encoding~\cite{havlicek_supervised_2019} require linear scaling of qubits with respect to the number of features. Alternatively, amplitude encoding provides logarithmic scaling in the number of qubits~\cite{schuld2018supervised}. However, without ancillary qubits, amplitude encoding results in deep circuits~\cite{nakaji_amplitude_2022}. In practice, when the feature space exceeds the capacity of available quantum hardware, classical dimensionality reduction algorithms are applied as a preprocessing step in quantum pipeline. Nevertheless, with ongoing advancements in quantum computing, biomarker discovery may eventually be performed without the need for classical preprocessing.

A recent benchmarking study~\cite{bowles2024better} provides a comprehensive evaluation of popular QML models on binary classification problems. The study examines QML architectures compatible with near term quantum devices such as quantum neural networks (QNNs), including quantum convolutional neural networks (QCNNs), and quantum kernel methods (QKMs).

The majority of QNNs are based on parametrized quantum circuits (PQCs). The parameters of PQCs are optimized using classical routines to minimize the problem’s loss function. A typical QNN begins with data embedding, followed by a series of unitary operations. One of the most general QNN models for classification is the Variational Quantum Classifier (VQC), which is essentially a PQC. Another example of a VQC is the circuit-centric quantum classifier~\cite{schuld_circuit-centric_2020}, one of the earliest proposed generic QNNs. Data re-uploading classifier is a notable QNN architecture that was shown to have universal approximation properties~\cite{perez-salinas_data_reup_2020}. The data re-uploading classifier features a processing layer composed of data encoding and unitary operations with trainable parameters. This layer is repeated $L$ times, each with independent parameters.

Recently, significant attention has been given to leveraging quantum computers for evaluating kernel functions in kernel methods. Quantum kernels, based on feature maps (data encodings), could be used with classical maximum margin classifiers. To evaluate a quantum kernel function, a circuit is designed by first applying a feature map and then its Hermitian conjugate. A prominent example of data-dependent quantum advantage in QML models is demonstrated through QKMs. The authors of the manuscript~\cite{huang_power_2021} established a relation between potential advantage in predictive accuracy of a model for a given dataset and a quantum kernel. In addition, a projected quantum kernel classifier was introduced.

%mention correspondance between QNNs and QKMs - example IQP classfier The IQP kernel classifier, inspired by IQP circuits that are challenging to simulate classically, is widely used in quantum machine learning.~\cite{havlicek_supervised_2019}

Although the predictive advantage of QML models for practically relevant problems remains an open question and necessitates data embeddings that are difficult to simulate classically, quantum models are expected to show better generalization than classical models, leveraging fewer data points~\cite{caro2022generalization}. This is particularly intriguing in fields where constructing sufficiently large datasets to ensure satisfactory performance of ML models is challenging.

The findings in Ref.~\cite{bowles2024better} highlight the significance of experimental design for quantum models’ performance. Problem-agnostic implementations of QML models are unlikely to outperform their classical counterparts. This observation implies that the embedding of classical data into Hilbert space and subsequent operations should be tailored to an application and available hardware. Another key finding is that reducing entanglement in quantum models may enhance algorithm performance. However, the observed behavior may be influenced by the data structure of the considered use cases. These insights underscore the importance of use case specific algorithm design for the potential benefits of quantum computing.

%maybe to cite in the text Universal expressiveness of variational quantum classifiers and quantum kernels for support vector machines Jonas Jäger & Roman V. Krems 

+QCNNs~\cite{qcnn}
+BP
+figure of QNNs, QKMs, data reuploading


\textbf{Dimensionality reduction using quantum computing methods.}  

As quantum computing rapidly develops, quantum algorithms for reducing the feature space size are evolving alongside it. For instance, many classical dimensionality reduction algorithms have a quantum adaptation, such as quantum linear discriminant analysis (QLDA)~\cite{yu_qLDA_2023}, quantum slow  feature analysis(QSFA)~\cite{kerenidis_classification_qSFA_2020}, quantum isomap (QIsomap) ~\cite{feng_qIsomap_2024}. However, the majority of the quantum algorithms for dimensionality reduction still require further technological advancements to achieve practical relevance.

Through the example of quantum principal component analysis (QPCA), we aim to illustrate how advancements in the field are shaping the potential advantages and algorithmic implementations. Utilized for feature extraction, QPCA was proposed in~\cite{lloyd_qPCA}, suggesting potential speedups in clustering and pattern recognition tasks. However, the proposed QPCA algorithm requires fault-tolerant hardware and raises concerns on validity of the assumptions to achieve an exponential speedup~\cite{qpca_state_assumptions}. 

%Although near term algorithms for QPCA are present in the literature~\cite{larose_var_state_diag_pca, resonant_qPCA}, the extent of the anticipated speed-ups remains uncertain. On the other hand, the QPCA speedup on quantum data is highlighted in~\cite{covariance_qPCA}.

\textbf{Somewhere refer to the figure}

\textbf{Regression using quantum computing.}
\begin{itemize}
    \item quantum linear regression~\cite{wiebe_quantum_fitting_2012, wang_quantum_regression_2017, zhao_quantum-assisted_gpr_2019, date_adiabatic_regression_2021}
\end{itemize}


\textbf{Clustering using quantum computing.}
\begin{itemize}
    \item Quantum k-Means~\cite{khan_qk-means_2019, arthur_balanced_k_means_2021}
    \item Quantum spectral clustering~\cite{kerenidis_quantum_spectral_2021}
\end{itemize}

%Raj to flesh out
\textbf{Generating data using quantum computing.}

\begin{itemize}
    \item Quantum neural networks (qNNs) - qCBMs~\cite{benedetti_generative_qcbm_2019}, qGANs
    \item Quantum Boltzmann Machines (qBMs)~\cite{amin_quantum_2018}
\end{itemize}



\begin{table}
    \centering
    \begin{tabular}{ m{4cm}  m{4cm} m{4cm} }
       Learning task  & Use case example & Quantum algorithm \\
    \hline
    \hline
         Dimensionality reduction & Identification of covariates for biomarker traits regression models & QPCA~\cite{lloyd_qPCA, larose_var_state_diag_pca, resonant_qPCA, covariance_qPCA}, QLDA~\cite{yu_qLDA_2023}, QSFA~\cite{kerenidis_classification_qSFA_2020}, QIsomap~\cite{feng_qIsomap_2024}\\
         Classification & Omics data, medical images, EHRs & QNNs~\cite{perez-salinas_data_reup_2020, qcnn, schuld_circuit-centric_2020}, QKMs~\cite{havlicek_supervised_2019, huang_power_2021} \\ 
         Regression & & quantum linear regression algorithms~\cite{wiebe_quantum_fitting_2012, wang_quantum_regression_2017, zhao_quantum-assisted_gpr_2019, date_adiabatic_regression_2021}\\
         Clustering & Omics data & quantum k-Means~\cite{khan_qk-means_2019, arthur_balanced_k_means_2021}, quantum spectral clustering~\cite{kerenidis_quantum_spectral_2021} \\
         Generative learning & & QNNs~\cite{benedetti_generative_qcbm_2019}, QBMs~\cite{amin_quantum_2018}\\ 
         Time series analysis & EHRs, longitudinal studies, identification of drug resistance mechanisms & quantum autoencoder \cite{sakhnenko2022hybrid}, quantum reservoir computing \cite{suzuki2022natural} \\
         Natural language processing & Clinical notes processing~\cite{singhal2023opportunities} & QLSTM~\cite{di2022dawn}, VQA~\cite{cer_qnlp_vqa_2018} \\ 
         Anomaly detection & & \\
         Optimization & & Quantum-behaved PSO \\
         \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


%\cite{guarasci2022quantum, di2022dawn}
%~\cite{singhal2023opportunities} 
%add quantum graph neural networks, random walks? - gene regulatory networks?, QTDA?, 
% B-cell differentiation circuit model -106, 107
